Localization in the Crowd with Topological Constraints

We address the problem of crowd localization, i.e., the prediction of dots corresponding to people in a crowded scene. Due to various challenges, a localization method is prone to spatial semantic errors, i.e., predicting multiple dots within a same person or collapsing multiple dots in a cluttered region. We propose a topological approach targeting these semantic errors. We introduce a topological constraint that teaches the model to reason about the spatial arrangement of dots. To enforce this constraint, we define a persistence loss based on the theory of persistent homology. The loss compares the topographic landscape of the likelihood map and the topology of the ground truth. Topological reasoning improves the quality of the localization algorithm especially near cluttered regions. On multiple public benchmarks, our method outperforms previous localization methods. Additionally, we demonstrate the potential of our method in improving the performance in the crowd counting task.

==> xsec-experiments.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\tabcolsep}{4pt}
% \begin{table*}[h]
\begin{table*}[h]
\small
\begin{center}
\begin{tabular}{|p{0.26\linewidth}|p{0.03\linewidth}|p{0.03\linewidth}|p{0.03\linewidth}|p{0.03\linewidth}|p{0.03\linewidth}|p{0.03\linewidth}|p{0.03\linewidth}|p{0.03\linewidth}|p{0.03\linewidth}|}

\hline
% \noalign{\smallskip}
 & \multicolumn{3}{p{0.13\linewidth}|}{\centering {ShanghaiTech A}}  & \multicolumn{3}{p{0.13\linewidth}|}{\centering {ShanghaiTech B}} & \multicolumn{3}{p{0.13\linewidth}|}{\centering {UCF QNRF}}\\
% \noalign{\smallskip}
\hline
% \noalign{\smallskip}
Model & \centering {G(1)}  & \centering {G(2)}  & \centering {G(3)}  & \centering {G(1)}  & \centering {G(2)}  & \centering {G(3)}  & \centering {G(1)}  & \centering {G(2)}  & \centering {G(3)} \cr 
\hline
CSRNet \cite{csr:cvpr:2018} 
    & \centering 76 & \centering 113 & \centering 149 
    & \centering 13 & \centering 21 & \centering 29 
    & \centering 157 & \centering 187 & \centering 219 \cr 
Bayesian \cite{bayesian:2019:ICCV} 
    & \centering 75 & \centering 90 & \centering 130 
    & \centering \textbf{10} & \centering \textbf{14} & \centering 23 
    & \centering \textbf{100} & \centering \textbf{117} & \centering 150 \cr 
LSC-CNN \cite{locate:LSC-CNN:babu:ipmi:2020} 
    & \centering 70 & \centering 95 & \centering 137 
    & \centering \textbf{10} & \centering 17 & \centering 27 
    & \centering 126 & \centering 160 & \centering 206 \cr 
TopoCount (ours)  
    & \centering \textbf{69} & \centering \textbf{81} & \centering \textbf{104}
    & \centering \textbf{10} & \centering \textbf{14} & \centering \textbf{20} 
    & \centering 102 & \centering 119  & \centering \textbf{148}\cr 

\hline
\end{tabular}
\caption{Grid Average Mean absolute Errors (GAME) }
\label{table:game}
\end{center}
\vspace{-.1in}
\end{table*}
\setlength{\tabcolsep}{1.4pt}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\small
% \parbox{.5\linewidth}{
\centering
\begin{tabular}{|p{0.3\linewidth}|p{0.18\linewidth}|p{0.2\linewidth}|p{0.2\linewidth}|}
% \begin{tabular}{|c|c|c|c|}
\hline
% \noalign{\smallskip}
% \centering {Method} & \centering {Avg. Prec.}  & \centering {Avg. Recall}  & \centering {Avg. F-score} \cr 
\centering {Method} & \centering {Prec.}  & \centering {Recall}  & \centering {F-score} \cr 
\hline
MCNN 
    % \cite{multicolumn:cc:cvpr:2016} 
    & \centering 59.93\% & \centering 63.50\% & \centering 61.66\% \cr 
CL-CNN D$_{\infty}$ 
    % \cite{qnrf:Idrees:CompositionLF:eccv:2018} 
    & \centering 75.8\% & \centering 59.75\% & \centering 66.82\% \cr 
LSC-CNN 
    % \cite{locate:LSC-CNN:babu:ipmi:2020} 
    & \centering 74.62\% & \centering 73.50\% & \centering 74.06\% \cr 
TopoCount 
    % (Ours)  
    & \centering \textbf{81.77}\% & \centering \textbf{78.96}\% & \centering \textbf{80.34}\% \cr 
\hline
\end{tabular}
\caption{Localization accuracy on the UCF QNRF dataset,  with metric in \cite{qnrf:Idrees:CompositionLF:eccv:2018}}
\label{table:f1score}
% }
\end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\tabcolsep}{4pt}
\begin{table}[h]
\small
\begin{center}
\begin{tabular}{|p{0.55\linewidth}|p{0.35\linewidth}|}

\hline
Method  & 
\centering {F1-m / Pre / Rec (\%)}  
\cr
\hline
\multirow{2}{*}{Faster RCNN \cite{fasterrcnn:nips:2015}}
    & \centering $\sigma_l:$ 6.7 / \textbf{95.8} / 3.5  \cr
    & \centering $\sigma_s:$ 6.3 / \textbf{89.4} / 3.3  
     \cr
\hline
\multirow{2}{*}{TinyFaces \cite{tinyfaces:cvpr:2017}} 
    & \centering  $\sigma_l:$ 56.7 / 52.9 / 61.1   \cr
    & \centering  $\sigma_s:$ 52.6 / 49.1 / 56.6  
     \cr
\hline
\multirow{2}{*}{VGG+GPR \cite{vgg:grp:gao2019domainadaptive}} 
    & \centering  $\sigma_l:$ 52.5 / 55.8 / 49.6    \cr
    & \centering  $\sigma_s:$ 42.6 / 45.3 / 40.2  
     \cr
\hline     

\multirow{2}{*}{RAZ\_Loc \cite{RAZ-Net:detect:cvpr:2019} }
    & \centering  $\sigma_l:$ 59.8 / 66.6 / 54.3   \cr
    & \centering $\sigma_s:$ 51.7 / 57.6 / 47.0   
    \cr
\hline    
\multirow{2}{*}{TopoCount (ours)  }
    & \centering  $\sigma_l:$ \textbf{69.1} / 69.5 / \textbf{68.7}   \cr
    & \centering  $\sigma_s:$ \textbf{60.1} / 60.5 / \textbf{59.8}   
    \cr
    
   
\hline
\end{tabular}
\caption{NWPU-Crowd Localization Challenge }
\label{table:nwpu}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Varying Lambda
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h!]
\small
\begin{center}
\begin{tabular}{|p{0.1\linewidth}|p{0.12\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|p{0.13\linewidth}|}
\hline

 & \centering BCE & \centering DICE  & \centering $\lambda=0.5$ & \centering $\lambda=1.0$ & \centering $\lambda=1.5$ & \centering $\lambda=2.0$   \cr 
\hline
 {G(3)}  & \centering 122 & \centering 114 & \centering 109 & \centering \textbf{104} & \centering  \textbf{104}
 & \centering 107 \cr 
\hline
\end{tabular}
\caption{Ablation study for the loss function. Compare the localization score G(3) on the ShanghaiTech A dataset of TopoMap trained with: (a) weighted BCE loss, (b) DICE loss ($\lambda=0$), (c) DICE and Persistence loss ($\lambda \in [0.5, 2]$). 
} 
\label{table:lambda_pers_vary_sh_a}
\end{center}
\vspace{-.15in}
\end{table}
\setlength{\tabcolsep}{1.4pt}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\tabcolsep}{4pt}
\begin{table}[h]
\small
\begin{center}
\begin{tabular}{|p{0.14\linewidth}|p{0.17\linewidth}|p{0.17\linewidth}|p{0.17\linewidth}|p{0.17\linewidth}|}

\hline
% \noalign{\smallskip}
 & \multicolumn{2}{p{0.35\linewidth}|}{\centering {ShanghaiTech A}}  &  \multicolumn{2}{p{0.35\linewidth}|}{\centering {UCF QNRF}}\\
% \noalign{\smallskip}
\cline{2-5}
% \noalign{\smallskip}
  &  \centering $\sigma=20$  & \centering $\sigma=5$  & \centering $\sigma=20$  & \centering $\sigma=5$   \cr 
% \hline
  & \centering {mAP/mAR} & \centering {mAP/mAR}   & \centering {mAP/mAR} & \centering {mAP/mAR}   \cr 
\hline
RAZ\_Loc 
    & \centering $58.4/74.1$ & \centering $19.7/42.2$
    & \centering $28.4/48.3$ & \centering $3.7/14.8$
    \cr 
TopoCount 
    & \centering $\textbf{85.0}/\textbf{82.8}$  & \centering $\textbf{56.0}/\textbf{54.8}$
    & \centering $\textbf{69.0}/\textbf{66.5}$  & \centering $\textbf{27.1}/\textbf{26.2}$
    \cr 

\hline
\end{tabular}
\caption{Localization accuracy using metric in \cite{RAZ-Net:detect:cvpr:2019}.}
\label{table:raz_metric}
\end{center}
\vspace{-.15in}
\end{table}
\setlength{\tabcolsep}{1.4pt}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% All CC Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \vspace{-0.5cm}
\setlength{\tabcolsep}{4pt}
\begin{table*}[t]
\small
\begin{center}
\begin{tabular}{|p{0.31\linewidth}|p{0.034\linewidth}|p{0.043\linewidth}|p{0.034\linewidth}|p{0.043\linewidth}|p{0.035\linewidth}|p{0.043\linewidth}|p{0.034\linewidth}|p{0.043\linewidth}|p{0.034\linewidth}|p{0.043\linewidth}|p{0.034\linewidth}|p{0.043\linewidth}|}

\hline
% \noalign{\smallskip}
 & \multicolumn{2}{p{0.092\linewidth}|}{\centering {Shanghai. A}}  & \multicolumn{2}{p{0.092\linewidth}|}{\centering {Shanghai. B}} & \multicolumn{2}{p{0.093\linewidth}|}{\centering {UCF CC 50}} & \multicolumn{2}{p{0.093\linewidth}|}{\centering {UCF QNRF}} &
 \multicolumn{2}{p{0.092\linewidth}|}{\centering {JHU++}} &
 \multicolumn{2}{p{0.092\linewidth}|}{\centering {NWPU}}\\
% \noalign{\smallskip}
\hline
% \noalign{\smallskip}
Model 
& \centering {MAE}  & \centering {RMSE}  
& \centering {MAE}  & \centering {RMSE}  
& \centering {MAE}  & \centering {RMSE}  
& \centering {MAE}  & \centering {RMSE}
& \centering {MAE}  & \centering {RMSE}
& \centering {MAE}  & \centering {RMSE}
\cr 
\hline
IC-CNN \cite{iterativeCC:Ranjan:eccv:2018} 
    & \centering 68.5 & \centering 116.2 
    & \centering 10.7 & \centering 16 
    & \centering 260.9 & \centering 365.5 
    & \centering - & \centering -
    & \centering - & \centering -
    & \centering - & \centering - 
    \cr 
CSRNet \cite{csr:cvpr:2018} 
    & \centering 68.2 & \centering 115 
    & \centering 10.6 & \centering 16 
    & \centering 266.1 & \centering 397.5 
    & \centering - & \centering -
    & \centering 85.9  & \centering 309.2
    & \centering 121.3 & \centering 387.8 
    \cr 
SANet \cite{sanet:eccv:2018} 
    & \centering 67 & \centering 104.5 
    & \centering 8.4 & \centering 13.6 
    & \centering 258.4 & \centering 334.9 
    & \centering - & \centering -
    & \centering 91.1  & \centering 320.4
    & \centering 190.6 & \centering 491.4 
    \cr 
ANF \cite{anf:iccv:2019} 
    & \centering 63.9 & \centering 99.4 
    & \centering 8.3 & \centering 13.2 
    & \centering 250.2 & \centering 340 
    & \centering 110 & \centering 174
    & \centering - & \centering -
    & \centering - & \centering - 
    \cr 
RAZ-Net \cite{RAZ-Net:detect:cvpr:2019} 
    & \centering 65.1 & \centering 106.7 
    & \centering 8.4 & \centering 14.1 
    & \centering - & \centering - 
    & \centering 116 & \centering 195
    & \centering - & \centering - 
    & \centering 151.5 & \centering 634.7 
    \cr  %related
LSC-CNN \cite{locate:LSC-CNN:babu:ipmi:2020} 
    & \centering 66.4 & \centering 117.0 
    & \centering 8.1 & \centering 12.7 
    & \centering 225.6 & \centering 302.7 
    & \centering 120.5 & \centering 218.2
    & \centering 112.7  & \centering 454.4 
    & \centering - & \centering - 
    \cr  % this paper ignores some sota methods in cc to show they get better count numbers
CAN \cite{canet:Liu:2019:CVPR} 
    & \centering 62.3 & \centering 100 
    & \centering 7.8 & \centering 12.2 
    & \centering 212.2 & \centering \textbf{243.7} 
    & \centering 107 & \centering 183
    & \centering 100.1  & \centering 314.0
    & \centering 106.3 & \centering \textbf{386.5} 
    \cr 
Bayesian \cite{bayesian:2019:ICCV} 
    & \centering 62.8 & \centering 101.8 
    & \centering 7.7 & \centering 12.7 
    & \centering 229.3 & \centering 308.2 
    & \centering \textbf{89} & \centering \textbf{155}
    & \centering 75.0  & \centering 299.9
    & \centering \textbf{105.4} & \centering 454.2 
    \cr 
CG-DRC \cite{sindagi2020jhu-crowd++:dataset} 
    & \centering 60.2 & \centering 94.0 
    & \centering \textbf{7.5} & \centering \textbf{12.1}
    & \centering - & \centering - 
    & \centering 95.5  & \centering 164.3 
    & \centering 71.0  & \centering 278.6 
    & \centering - & \centering - 
    \cr  %related
ASNet \cite{attention-scaling:jiang:2020:CVPR} 
    & \centering \textbf{57.8} & \centering \textbf{90.1} 
    & \centering - & \centering - 
    & \centering \textbf{174.8}  & \centering 251.6 
    & \centering 91.6  & \centering 159.7
    & \centering - & \centering - 
    & \centering - & \centering - 
    \cr 

\hline

TopoCount (Ours)
    & \centering 61.2 & \centering 104.6 
    & \centering 7.8 & \centering 13.7 
    & \centering 184.1 & \centering 258.3 
    & \centering \textbf{89} & \centering 159
    & \centering \textbf{60.9} & \centering \textbf{267.4} 
    & \centering 107.8 & \centering 438.5 
    \cr % \noalign{\smallskip} % Q epoch 75 - 0.4-0.5 % parta e84 0.4-0.5 % partb e84 0.4-0.5

\hline

\hline
\end{tabular}
\caption{Counting Performance Evaluation}
\label{table:cc_all}
\end{center}
\end{table*}
\setlength{\tabcolsep}{1.4pt}
% \vspace{-0.8cm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\setlength{\tabcolsep}{4pt}
\begin{table*}[h]
\small
\begin{center}
\begin{tabular}{|p{0.27\linewidth}|p{0.054\linewidth}|p{0.054\linewidth}|p{0.054\linewidth}|p{0.054\linewidth}|p{0.054\linewidth}|p{0.054\linewidth}|p{0.054\linewidth}|p{0.054\linewidth}|p{0.054\linewidth}|p{0.054\linewidth}|}

\hline
% \noalign{\smallskip}
 & \multicolumn{2}{p{0.12\linewidth}|}{\centering {ShanghaiTech A}}  & \multicolumn{2}{p{0.12\linewidth}|}{\centering {ShanghaiTech B}} & \multicolumn{2}{p{0.12\linewidth}|}{\centering {UCF CC 50}} & \multicolumn{2}{p{0.12\linewidth}|}{\centering {UCF QNRF}} &
 \multicolumn{2}{p{0.12\linewidth}|}{\centering {JHU++}}\\
% \noalign{\smallskip}
\hline
% \noalign{\smallskip}
Model & \centering {MAE}  & \centering {RMSE}  & \centering {MAE}  & \centering {RMSE}  & \centering {MAE}  & \centering {RMSE}  & \centering {MAE}  & \centering {RMSE}& \centering {MAE}  & \centering {RMSE}\cr 
\hline


CAN \cite{canet:Liu:2019:CVPR} 
    & \centering 62.3 & \centering 100 
    & \centering 7.8 & \centering \textbf{12.2} 
    & \centering 212.2 & \centering \textbf{243.7} 
    & \centering 107 & \centering 183
    & \centering 100.1 & \centering 314.0 
    \cr 


TopoCount + CAN (Ours)
    & \centering \textbf{59.5 \\ \textit{-4.5\%} }  & \centering \textbf{93.3 \\ \textit{-6.7\%}}  
    & \centering  \textbf{7.5 \\ \textit{-2.5\%}} & \centering 13.2 \\ \textit{+8.1\%}
    & \centering \textbf{190 \\ \textit{-10.5\%}} & \centering 249 \\ \textit{+2.2\%}
    & \centering \textbf{99  \\ \textit{-7.5\%}}& \centering \textbf{162  \\ \textit{-11.5\%}}
    & \centering \textbf{71.9\\ \textit{-28.2\%}} & \centering \textbf{260.9 \\ \textit{-19.9\%}}
    \cr
\hline
% \hline
Bayesian \cite{bayesian:2019:ICCV} 
    & \centering 62.8 & \centering 101.8 
    & \centering 7.7 & \centering 12.7 
    & \centering 229.3 & \centering 308.2 
    & \centering 89 & \centering 155
    & \centering 75.0 & \centering 299.9 
    \cr 

TopoCount + Bayesian (Ours)
    & \centering \textbf{58 \\ \textit{-7.6\%}}  & \centering \textbf{96.3 \\ \textit{-5.4\%}}  
    & \centering  \textbf{7.2 \\ \textit{-6.5\%}}  & \centering \textbf{11.8 \\ \textit{-7.1\%}} 
    & \centering \textbf{191 \\ \textit{-16.7\%}}  & \centering \textbf{257 \\ \textit{-16.6\%}}  
    & \centering \textbf{85 \\ \textit{-4.5\%}}  & \centering \textbf{148 \\ \textit{-4.5\%}} 
    & \centering \textbf{61.8 \\ \textit{-17.6\%}} & \centering \textbf{262.0 \\ \textit{-12.7\%}} 
    \cr
    


\hline

\hline
\end{tabular}
\caption{Integration of TopoMap with density estimation methods.}
\label{table:integration}
\end{center}
\end{table*}
\setlength{\tabcolsep}{1.4pt}
% \vspace{-0.8cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We validate our method on popular and large scale crowd counting benchmarks including ShanghaiTech parts A and B \cite{multicolumn:cc:cvpr:2016}, UCF CC 50 \cite{ucfcc50:idrees:cvpr:2013}, UCF QNRF \cite{qnrf:Idrees:CompositionLF:eccv:2018}, JHU++ \cite{sindagi2020jhu-crowd++:dataset}, and NWPU Challenge \cite{gao:nwpu:tpmi:2020}.

For the localization task, our method is superior compared to other methods. Moreover, we show that the localization results of our method benefits the counting task.

\myparagraph{Training Details.}
We train our \emph{TopoCount} with the dilated ground truth dot mask. The dilation is by default up to 7 pixels. 
For JHU++ and NWPU, which are provided with head box annotation, we use a more accurate dilation guided by the box size, $\max$(7, box width/2, box height/2). In all cases the dilation is no more than half the distance to the nearest neighbor to avoid overlapping of nearby dots. 

 The window size of the patch for topological constraint controls the level of localization we would like to focus on. \myhighlight{Since the scale of persons within an image is highly heterogeneous, varying the window size based on scale sounds intriguing. However the ground truth dot annotation generally do not carry scale information. As a result, we fix the patch size for each dataset.}
 We empirically choose $50{\times}50$ pixels patches for ShanghaiTech and UCF CC 50, and  $100{\times}100$ pixels patches for the larger scale datasets UCF QNRF, JHU++, and NWPU to account for the larger scale variation. An ablation study on the patch size selection is in the \textit{supplemental material}. The persistence loss is applied on grid tiles to enforce topological consistency between corresponding prediction and ground truth tiles/patches. Coordinates of the top left corner of the grid are randomly perturbed to prevent training with fixed tiles and act as data augmentation. \myhighlight{It should be noted that this tiling procedure is only performed during training with the persistence loss and is not performed during inference.}

The model is trained with the combined loss $L$ (Eq.~\eqref{eqn:total-loss}). During the first few epochs the likelihood map is random and is not topologically informative. Thus, in the beginning of training we use DICE loss only ($\lambda = 0$). When the model starts to converge to reasonable likelihood maps, we add the persistence loss with  $\lambda = 1.0$. Fig.~\ref{fig:test_4cc} shows qualitative results. More sample results are in the \textit{supplemental material}. 

\subsection{Localization Performance}
We evaluate \emph{TopoCount} on several datasets using (1) localized counting; (2) F1-score matching accuracy; and (3) the NWPU localization challenge metric.

\myparagraph{Localized Counting.}
We evaluate the counting performance within small grid cells and aggregate the error. The Grid Average Mean absolute Errors (GAME) metric \cite{game:trancos:2015:IbPria}, $G(L)$, divides the image into $4^L$ non-overlapping cells.
In Table~\ref{table:game}, the cell count in the localization-based methods LSC-CNN \cite{locate:LSC-CNN:babu:ipmi:2020} and TopoCount is the sum of predicted dots in the cell. On the other hand, the cell count in the density map estimation methods CSRNet \cite{csr:cvpr:2018} and Bayesian \cite{bayesian:2019:ICCV} is the integral
of the density map over the cell area. TopoCount achieves
the lowest error especially at the finest scale (level L=3), which indicates higher localization accuracy by the predicted dots.

\myparagraph{Matching Accuracy.}
We evaluate matching accuracy in two ways. First, similar to 
\cite{qnrf:Idrees:CompositionLF:eccv:2018} on the UCF QNRF dataset, we perform a greedy matching between detected locations and ground truth dots at thresholds varying from 1 to 100 and average the precision, recall, and F-scores over all thresholds. We compare with scores reported in \cite{qnrf:Idrees:CompositionLF:eccv:2018} in addition to calculated scores for SOTA localization methods \cite{locate:LSC-CNN:babu:ipmi:2020}.  
Table \ref{table:f1score} shows that our method achieves the highest F-score. 

Second, similar to \cite{RAZ-Net:detect:cvpr:2019} on ShanghaiTech Part A and UCF QNRF datasets, we impose at each dot annotation an un-normalized Gaussian function parameterized by $\sigma$. A true positive is a predicted dot whose response to the Gaussian function is greater than a threshold $t$. We compare with \cite{RAZ-Net:detect:cvpr:2019} results at $\sigma=5$ and $\sigma=20$. Table~\ref{table:raz_metric} reports the mean average precision (mAP) and mean average recall (mAR) for $t \in [0.5, 0.95]$, with a step of $0.05$. TopoCount achieves the highest scores with a large margin at both the small and large sigma $\sigma$.

\myparagraph{NWPU-Crowd Online Localization Challenge.}
NWPU dataset provides dot annotation in addition to box coordinates with specified width, $w$, and height, $h$, surrounding each head. The online challenge evaluates the F-score with 2 adaptive matching distance thresholds: $\sigma_l=\sqrt{w^2+h^2}/2$ and a more strict threshold $\sigma_s=min(w, h)/2$. Table \ref{table:nwpu} shows the F-score, precision, and recall with the 2 thresholds against the published challenge leaderboard. TopoCount achieves the highest F-score in both thresholds. More results are in the \textit{supplemental material}. 

\myparagraph{Ablation Study for the Loss Function.}
On the ShanghaiTech Part A dataset, we compare the performance of TopoCount trained with variations of the loss function in Eq.~\ref{eqn:total-loss}: (1) per-pixel weighted Binary Cross Entropy (BCE) loss as in \cite{RAZ-Net:detect:cvpr:2019} with empirically chosen weight of 5 to account for the amount of class imbalance in the ground truth dot maps, (2) per-pixel DICE loss only (i.e $\lambda=0$ in Eq.~\ref{eqn:total-loss}), and (3) a combined per-pixel DICE loss and Persistence loss with $\lambda \in \{0.5,1,1.5,2\}$. 
The results in Table \ref{table:lambda_pers_vary_sh_a} show the
training with BCE loss gives the largest error. With $\lambda=0$, i.e., DICE without the persistence loss, the error is lower. The error is further lowered with the introduction of the persistence loss. Varying $\lambda$ between $0.5$ and $2.0$ the results are more robust and comparable, with the best performance at $\lambda = 1$ and $\lambda = 1.5$. Consequently, we use $\lambda = 1$ in all our experiments.


\subsection{Counting Performance}
Our localization method can be directly applied to crowd counting task. 
It performs competitively among SOTA counting methods.
In Table~\ref{table:cc_all}, we compare TopoCount's overall count in terms of the Mean Absolute Error (MAE) and Root Mean Squared Error (RMSE) against SOTA counting methods. Our method achieves SOTA performance on the new JHU++ large scale dataset and is mostly between second and third place for the other datasets compared to SOTA density-based methods. More detailed results on the JHU++ are in the \textit{supplemental material}.


\myparagraph{Integration with Density-Based Methods.}
A high quality localization model can be combined with density-based methods to boost their performance. As described in Section~\ref{sec:method-integration}, we integrate TopoCount with two SOTA density-based counting algorithms and report the results.
Table~\ref{table:integration} shows that the integration results in a significant improvement over the individual performance of the density map models. This further demonstrates the high quality of TopoCount localization and suggests that more sophisticated density map models can benefit from high quality localization maps to achieve an even better counting performance.


